Online Market Equilibrium with Application to Fair Division

Computing market equilibria is a problem of both theoretical and applied interest. Much research to date focuses on the case of static Fisher markets with full information on buyers' utility functions and item supplies. Motivated by real-world markets, we consider an online setting: individuals have linear, additive utility functions; items arrive sequentially and must be allocated and priced irrevocably. We define the notion of an online market equilibrium in such a market as time-indexed allocations and prices which guarantee buyer optimality and market clearance in hindsight. We propose a simple, scalable and interpretable allocation and pricing dynamics termed as PACE. When items are drawn i.i.d. from an unknown distribution (with a possibly continuous support), we show that PACE leads to an online market equilibrium asymptotically. In particular, PACE ensures that buyers' time-averaged utilities converge to the equilibrium utilities w.r.t. a static market with item supplies being the unknown distribution and that buyers' time-averaged expenditures converge to their per-period budget. Hence, many desirable properties of market equilibrium-based fair division such as no envy, Pareto optimality, and the proportional-share guarantee are also attained asymptotically in the online setting. Next, we extend the dynamics to handle quasilinear buyer utilities, which gives the first online algorithm for computing first-price pacing equilibria. Finally, numerical experiments on real and synthetic datasets show that the dynamics converges quickly under various metrics.

==> texts-arxiv/abstract.tex <==
\begin{abstract}
    Computing market equilibria is a problem of both theoretical and applied interest. Much research focuses on the static case, but in many markets items arrive sequentially and stochastically. We focus on the case of online Fisher markets: individuals have linear, additive utility and items drawn from a distribution arrive one at a time in an online setting. We define the notion of an equilibrium in such a market and provide a dynamics which converges to these equilibria asymptotically. An important use-case of market equilibria is the problem of fair division. With this in mind, we show that our dynamics can also be used as an online item-allocation rule such that the time-averaged allocations and utilities converge to those of a corresponding static Fisher market. This implies that other good properties of market equilibrium-based fair division such as no envy, Pareto optimality, and the proportional share guarantee are also attained in the online setting. An attractive part of the proposed dynamics is that the market designer does not need to know the underlying distribution from which items are drawn. We show that these convergences happen at a rate of $O((\log t)/t)$ or $O((\log t)^2/t)$ in theory and quickly in real datasets.
\end{abstract}
    

==> texts-arxiv/conclusions.tex <==
% moved to experiments

% \section{Conclusion}
% We introduced the concept of an online Fisher market and proposed the PACE dynamics. We showed that when items arrive sequentially and stochastically, PACE converges to equilibrium outcomes of the underlying market model. 
% Furthermore, we showed that, as a consequence of this, PACE can be used in online fair division problems to generate an online allocation that, asymptotically, achieves the compelling fairness properties of CEEI.

% Many questions remain for future research. We mostly focused on the case where budgets are faux currency and there are many open questions for adapting PACE to a real-money budget-management setting as well as more complicated nonlinear utility models. Another imperative question, especially for practitioners, is whether PACE guarantees some level of incentive-compatibility.
% %In summary, online allocation with fairness and efficiency objectives is an exciting and practically important area for future work.

==> texts-arxiv/extensions.tex <==
\section{Extension to a continuum of items} \label{sec:extension}
In this section, we briefly discuss the extension of the above market dynamics to an ``infinite-dimensional'' Fisher market of a continuum of items \cite{gao2020infinite}. \cite{gao2020infinite} study convex programs to compute offline equilibrium quantities. Here, we view the continuum of items as an unknown item distribution from which items are sampled.

First, note that Algorithm \ref{alg:da} does not require a finite support of the random variable $z$, that is, we can choose any $\mathcal{Z}$ and a distribution $\mathcal{D}$ on $\mathcal{Z}$, as long as (i) we can sample $z_t$ from $\mathcal{D}$ and (ii) we can construct a subgradient of the ``sampled'' function $g^t = g_{z_t}(w^t) \in \partial f_t(w^t)$ (where $f_t = f_{z_t}$ and $g_z(w)$ is a subgradient oracle). In Theorem \ref{thm:general-conv}, we need $\sup_t \EE \|g^t\|^2 <\infty$, which holds as long as 
\[ \EE_{z\sim \mathcal{D}} \|g_z(w)\| < \infty. \]
Hence, in \S \ref{sec:conv-analysis-pace}, we can replace the set of items $[m]$ by another finite measure space, such as a compact subset of $\RR^d$. 

Next, we briefly recap the setup in \cite{gao2020infinite} in order to describe the extension. 
Let there be $n$ buyers and let $\Theta\subseteq \RR^d$ be a compact set representing the item space with unit (Lebesgue) measure $\mu(\Theta)=1$.\footnote{In fact, this also includes the case of $m$ items as a special case: if $\Theta = [m]$, let the measure be $\mu(A) = \frac{|A|}{m}$ for all $A\subseteq [m]$.}
Buyers' valuations $v_i$, as well as prices of items $p$, are nonnegative $L_1$ functions on $\Theta$, i.e., $v_i \in L_1(\Theta)_+$ and $p\in L_1(\Theta)_+$. An allocation is a set of bundles $x = (x_i)$, where each $x_i$ is an $L_\infty$ function on $\Theta$, i.e., $p\in L_1(\Theta)_+$. The supplies of all items is $\ones$, the constant function of value $1$ on $\Theta$. In \cite[\S 3]{gao2020infinite}, the authors give (infinite-dimensional) Eisenberg-Gale-type convex programs and show that they capture market equilibria of the infinite-dimensional Fisher market. The counterpart of \eqref{eq:eg-dual-p-beta} in the infinite-dimensional case is 
\[ \min_{\beta\in [B_i / (1+\delta_0), (1+\delta_0)\ones]} \langle \max_i \beta_i v_i, \ones \rangle - \sum_i B_i \log \beta_i, \]
where the notation $\langle a, b\rangle := \int_\Theta a b d\mu$ denotes applying the linear functional $b\in L_\infty(\Theta)$ on the vector $a\in L_1(\Theta)$. As shown in \cite[\S 3]{gao2020infinite}, the above convex program has a unique optimal solution $\beta^*$ corresponding to the equilibrium utility prices and $p^* = \max_i \beta^*_i v_i \in L_1(\Theta)_+$ gives equilibrium prices. Note that the first term $f(\beta) := \langle \max_i \beta_i v_i, \ones \rangle = \EE_\theta[f_\theta(\beta)]$, where $f_\theta(\beta) = \max_i \beta_i v_i(\theta)$ and the expectation is taken over $\theta\sim \mathcal{U}(\Theta)$, the uniform distribution on $\Theta$. 

For any (fixed) $\theta\in \Theta$, a subgradient of $f_\theta(\beta)$ is $g_\theta(\beta) = v_{i^*}(\theta) e^{(i^*)} \in \partial f_\theta(\beta)$. Similarly, by the additivity/linearity of subgradient, for any $\beta>0$,
\[ \EE_\theta g_\theta(\beta) \in \partial f(\beta). \]
In this case, Algorithm \ref{alg:da} leads to the same dynamics as noted in \cite[\S 3]{gao2020infinite}: starting from $\bar{g}^0 = 0$, $\beta^0 \in (B/(1+\delta_0), (1+\delta_0) \ones)$, at time step $t$,
\begin{enumerate}
    \item An item $\theta_t \sim \mathcal{U}(\Theta) $ is sampled independently, which gives a winner $i_t = \min \argmax \beta^t_i v_i(\theta_t)$. 
    \item Steps \ref{item:pace-buyer-bid-step}-\ref{item:pace-update-beta-step} remain unchanged, with all $j_t$ replaced by $\theta_t$.
\end{enumerate}

The convergence results, i.e., Theorems~\ref{thm:conv-beta(t)}-\ref{thm:asymp-envy-free} follow from similar arguments, as long as $\|v_i\|_\infty < \infty$ for all $i$. Here, the $\infty$-norm is understood as $\|v_i\|_\infty := \inf \{ M > 0: |v_i|\leq M\, {\rm a.e.} \}$, where {\rm a.e.} stands for almost everywhere, i.e., the preimage $\{\theta\in \Theta: |v_i(\theta)| \leq M \}$ has measure $1$.

% For quasilinear utilities, it is known that a market equilibrium can be captured by another primal-dual pair of convex programs \cite[\S Lemma 5]{cole2017convex}. Algorithm \eqref{alg:da} can be applied to a similar convex program too. \yuan{Should we mention the QL case at all...this discussion might be too raw/primitive.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

